S-Matrix for AdS from General Boundary QFT

The General Boundary Formulation (GBF) is a new framework for studying quantum theories. After concise overviews of the GBF and Schr\"odinger-Feynman quantization we apply the GBF to resolve a well known problem on Anti-deSitter spacetime where due to the lack of temporally asymptotic free states the usual S-matrix cannot be defined. We construct a different type of S-matrix plus propagators for free and interacting real Klein-Gordon theory.

==> zzzzz_head_packs_hyphs_iop.tex <==

\newcommand{\repa}{\RequirePackage}

\makeatletter\@ifpackageloaded{fixltx2e}{}{\repa{fixltx2e}}\makeatother
% provides some fixes to LaTeX2e, and the \TextOrMath command

\makeatletter\@ifpackageloaded{savesym}{}{\repa{savesym}}\makeatother
% There are a number of symbols that are defined by multiple packages.
% \savesymbol{XXX} renames a symbol from \XXX to \origXXX
% \restoresymbols{yyy}{XXX} renames \origXXX back to \XXX,
% and renames the current version of \XXX as \yyyXXX,
% see below at package stmaryrd for examples

\makeatletter\@ifpackageloaded{ae}{}{\repa{ae}}\makeatother

\makeatletter\@ifpackageloaded{amsfonts}{}{\repa{amsfonts}}\makeatother
\makeatletter
\@ifpackageloaded{amsmath}{\PassOptionsToPackage{intlimits}{amsmath}}
	{\repa[intlimits]{amsmath}}\makeatother
\makeatletter\@ifpackageloaded{amssymb}{}{\repa{amssymb}}\makeatother
\makeatletter\@ifpackageloaded{amsxtra}{}{\repa{amsxtra}}\makeatother

\makeatletter\@ifpackageloaded{array}{}{\repa{array}}\makeatother
\makeatletter\@ifpackageloaded{babel}{}{\repa[english]{babel}}\makeatother
\makeatletter\@ifpackageloaded{bbm}{}{\repa{bbm}}\makeatother
%\makeatletter\@ifpackageloaded{bibspacing}{}{\repa{bibspacing}}\makeatother
% sets space between bibliography items to zero

\makeatletter\@ifpackageloaded{calc}{}{\repa{calc}}\makeatother
\makeatletter\@ifpackageloaded{cancel}{}{\repa{cancel}}\makeatother
%\repa {color} % replaced by xcolor
\makeatletter\@ifpackageloaded{colordvi}{}{\repa{colordvi}}\makeatother
\makeatletter\@ifpackageloaded{colortbl}{}{\repa{colortbl}}\makeatother

\makeatletter\@ifpackageloaded{dsfont}{}{\repa{dsfont}}\makeatother
\makeatletter\@ifpackageloaded{empheq}{}{\repa{empheq}}\makeatother
\makeatletter\@ifpackageloaded{esint}{}{\repa{esint}}\makeatother
\makeatletter\@ifpackageloaded{eurosym}{}{\repa{eurosym}}\makeatother

\makeatletter\@ifpackageloaded{fancybox}{}{\repa{fancybox}}\makeatother
%\makeatletter\@ifpackageloaded{fancyhdr}{}{\repa{fancyhdr}}\makeatother
\makeatletter\@ifpackageloaded{float}{}{\repa{float}}\makeatother
\makeatletter\@ifpackageloaded{floatflt}{}{\repa{floatflt}}\makeatother
\makeatletter\@ifpackageloaded{fontenc}{}{\repa[OT2,T1]{fontenc}}\makeatother
\makeatletter\@ifpackageloaded{graphicx}{}{\repa{graphicx}}\makeatother

\makeatletter\@ifpackageloaded{hhline}{}{\repa{hhline}}\makeatother
\makeatletter\@ifpackageloaded{ifthen}{}{\repa{ifthen}}\makeatother
% contains \ifthenelse{test}{if-code}{else-code}

%\repa {indentfirst}
%\makeatletter\@ifpackageloaded{inputenc}{}{\repa[latin1]{inputenc}}\makeatother
\makeatletter\@ifpackageloaded{inputenc}{}{\repa[UTF8]{inputenc}}\makeatother

\makeatletter\@ifpackageloaded{lamsarrow}{}{\repa{lamsarrow}}\makeatother
\makeatletter\@ifpackageloaded{latexsym}{}{\repa{latexsym}}\makeatother
\makeatletter
\@ifpackageloaded{letterspace}{}{\repa[letterspace=10]{letterspace}}
\makeatother
% \textls[#1]{#2} prints text #2 with letterspacing #1 times 1/1000em
% \lsstyle changes letterspacing to letterspace=10 within group

\makeatletter\@ifpackageloaded{longtable}{}{\repa{longtable}\setlongtables}\makeatother 
% if problems with longtables occur, delete .aux file,
% or run twice without \setlongtables

%\repa {mathabx} 		% not used, because produces ugly \leq and \geq
%\makeatletter\@ifpackageloaded{mathbbol}{}{\repa{mathbbol}}\makeatother

\makeatletter
\@ifpackageloaded{makeidx}{}{\repa{makeidx}\makeindex}\makeatother
\makeatletter\@ifpackageloaded{mathtools}{}{\repa{mathtools}}\makeatother
%\makeatletter\@ifpackageloaded{microtype}{}{\repa{microtype}}\makeatother

%\repa {minitoc}
% called in zzzzz_head_book because not wanted in articles

%\repa {multicol}		% does not work with revtex
\makeatletter
\@ifpackageloaded{pb-diagram}{}{\repa{pb-diagram}}\makeatother
\makeatletter\@ifpackageloaded{pb-lams}{}{\repa{pb-lams}}\makeatother

\makeatletter\@ifpackageloaded{protosem}{}{\repa{protosem}}\makeatother

\makeatletter\@ifpackageloaded{slashed}{}{\repa{slashed}}\makeatother

\savesymbol{bigtriangleup}% save the original Latex 2e version
\savesymbol{bigtriangledown} % of \bigtriangleup as \origbigtriangleup
\makeatletter\@ifpackageloaded{stmaryrd}{}{\repa{stmaryrd}}\makeatother
\restoresymbol{stmaryrd}{bigtriangleup}
\restoresymbol{stmaryrd}{bigtriangleup}
% restore original version of \bigtriangleup,
% save the St. Mary Road version as \stmaryroadbigtriangleup

\makeatletter\@ifpackageloaded{subfigure}{}{\repa{subfigure}}\makeatother
%\makeatletter\@ifpackageloaded{t1enc}{}{\repa{t1enc}}\makeatother

\makeatletter\@ifpackageloaded{theorem}{}{\repa{theorem}}\makeatother
\makeatletter\@ifpackageloaded{ulem}{}{\repa{ulem}\normalem}\makeatother % \uwave, \dashuline, \dotuline \sout, \xout

\makeatletter\@ifpackageloaded{undertilde}{}{\repa{undertilde}}\makeatother
\makeatletter\@ifpackageloaded{upgreek}{}{\repa{upgreek}}\makeatother
% upright greek letters, e.g.: \uplambda, \Uplambda
% use: e.g. upright \phi for fields, normal (italic) \phi for angles

\makeatletter\@ifpackageloaded{verbatim}{}{\repa{verbatim}}\makeatother
\makeatletter\@ifpackageloaded{wasysym}{}{\repa{wasysym}}\makeatother
\makeatletter\@ifpackageloaded{wrapfig}{}{\repa{wrapfig}}\makeatother

\makeatletter\@ifpackageloaded{xcolor}{}{\repa{xcolor}}\makeatother

\makeatletter\@ifpackageloaded{xspace}{}{\repa{xspace}}\makeatother
% \xspace command
\makeatletter\@ifpackageloaded{yhmath}{}{\repa{yhmath}}\makeatother
%\makeatletter\@ifpackageloaded{hyperref}{}{\repa{hyperref}}\makeatother

\hyphenation{Min-kows-ki Schr\"o-din-ger eigen-value eigen-values}


